Ammonia, Methane, Hydrogen and Methanol Produced in Remote Renewable Energy Hubs: a Comparative Quantitative Analysis

Remote renewable energy hubs (RREHs) for synthetic fuel production are engineering systems harvesting renewable energy where it is particularly abundant. They produce transportable synthetic fuels for export to distant load centers. This article aims to evaluate the production costs of different energy carriers, and includes a discussion on advantages and disadvantages in terms of technical performance. To do so, we extend the study of Berger et al., (2021) which focuses on methane (CH4) as energy carrier and introduce three new carriers: ammonia (NH3), hydrogen (H2) and methanol (CH3OH). The four different RREHs are located in the Algerian Sahara desert and must serve to the load center, Belgium, a constant electro-fuel demand of 10 TWh per year. The modelling and optimisation of these systems are performed using the modelling language GBOML (Graph-Based Optimisation Modelling Language). Our findings reveal that the three new RREHs, each with its respective carrier (ammonia, hydrogen, and methanol), are all more cost-effective than the methane-based system. Ammonia demonstrates the most favourable cost-to-energy exported ratio.

==> 00-header-footer.tex <==
\pagestyle{scrheadings}
\titlehead{\vspace*{-2cm}\includegraphics[width=3.2cm]{fig/ecos-2024-logo.jpg}}
\ohead{\textit{Paper ID: 233}, Page \pagemark}
\cfoot{\color{gray}37\textsuperscript{th} INTERNATIONAL CONFERENCE ON EFFICIENCY, COST, OPTIMIZATION, SIMULATION AND ENVIRONMENTAL IMPACT OF ENERGY SYSTEMS, 30 JUNE -- 4 JULY, 2024, RHODES, GREECE}

==> 00-title-abstract.tex <==
\title{AMMONIA, METHANE, HYDROGEN AND METHANOL PRODUCED IN REMOTE RENEWABLE ENERGY HUBS: A COMPARATIVE QUANTITATIVE ANALYSIS}
\author[1, \ddag]{Antoine Larbanois}
\author[1, *, \ddag]{Victor Dachet}
\author[1]{Antoine Dubois}
\author[1]{Raphaël Fonteneau}
\author[1,2]{Damien Ernst}
\affil[1]{Department of Computer Science and Electrical Engineering, Liege University, Liege, Belgium}
\affil[2]{LTCI, Telecom Paris, Institut Polytechnique de Paris, Paris, France}




\ca{*Corresponding Author: victor.dachet@uliege.be}

\maketitle	

\section*{ABSTRACT}
Remote renewable energy hubs (RREHs) for synthetic fuel production are engineering systems harvesting renewable energy where it is particularly abundant. They produce transportable synthetic fuels for export to distant load centers. This article aims to evaluate the production costs of different energy carriers, and includes a discussion on advantages and disadvantages in terms of technical performance. To do so, we extend the study of \citet{berger2021remote} which  focuses on methane (CH$_4$) as energy carrier and introduce three new carriers: ammonia (NH$_3$), hydrogen (H$_2$) and methanol (CH$_3$OH). The four different RREHs are located in the Algerian Sahara desert and must serve  to the load center, Belgium, a constant electro-fuel demand of 10 TWh per year. The modelling and optimisation of these systems are performed using the modelling language GBOML (Graph-Based Optimisation Modelling Language). Our findings reveal that the three new RREHs, each with its respective carrier (ammonia, hydrogen, and methanol), are all more cost-effective than the methane-based system. Ammonia demonstrates the most favourable cost-to-energy exported ratio.

\def\thefootnote{\ddag}\footnotetext{These authors contributed equally to this work.}


==> tableau.tex <==
\begin{table*}[ht!]
\begin{tabularx}{\textwidth}{c|c|c|c|c}
  RREH & $CH_4$ & $CH_3OH$ & $H_2$ & $NH_3$\\
\hline 
$\mathcal{L}$ &  \multicolumn{4}{c}{Sahara Desert, Algerian Coast, Belgium} \\
\hline
$\mathcal{G}$ &  \multicolumn{4}{c}{All Technologies and commodity flows are represented in \autoref{fig:All_RREHs}}\\
\hline
$\mathcal{C}$ &  \begin{tabular}[l]{@{}l@{}}Electricity, $H_2$, $H_2O$, \\ $CO_2$, and $CH_4$\end{tabular}  & \begin{tabular}[l]{@{}l@{}}Electricity, $H_2$, $H_2O$,\\  $CO_2$, and $CH_3OH$\end{tabular} &  \begin{tabular}[l]{@{}l@{}}Electricity, $H_2$, \\ $H_2O$\end{tabular} & \begin{tabular}[l]{@{}l@{}}Electricity, $H_2$, $H_2O$, $N_2$, and \\$NH_3$\end{tabular} \\
\hline
$\mathcal{I}$ &  \multicolumn{4}{c}{\begin{tabular}[c]{@{}c@{}}These hubs does not need any direct import or exchange from another systems. \\ Their feed stocks are air and sea water.\end{tabular}}\\ 
\hline
$\mathcal{E}$ &  $CH_4$   &  $CH_3OH$   &  $H_2$  & $NH_3$\\
\hline
$\mathcal{B}$ & \multicolumn{3}{|c|}{\begin{tabular}[|c|]{@{}l@{}}Heat and Oxygen. Where the heat is generated by exothermic \\ process and the oxygen comes from PEM electrolyser\end{tabular}}                                                                            & \begin{tabular}[|c|]{@{}l@{}}In addition to heat and oxygen, a third by-product  \\ is argon. Which is produced by the ASU.\end{tabular}\\ 
\hline
$\mathcal{O}$ &  \multicolumn{3}{|c|}{\begin{tabular}[c]{@{}c@{}}The integration of desalination units within urban \\ water supply networks ensures a dependable source of drinking water, \\ even in the face of changing climate patterns and population growth.\end{tabular}} & \begin{tabular}[c]{@{}c@{}}In addition to the desalination unit, \\ the generated ammonia can contribute \\ to the development of local agriculture.\end{tabular}

\end{tabularx}
\end{table*}





\begin{table*}[ht!]
\centering
\begin{tabular}{p{1cm}|p{3cm}|p{3cm}|p{3cm}|p{3cm}}
RREH & Methane & Methanol & Hydrogen & Ammonia\\
\hline 
$\mathcal{L}$ &  \multicolumn{4}{p{12cm}}{Sahara Desert, Algerian Coast, Belgium} \\
\hline
$\mathcal{G}$ &  \multicolumn{4}{p{12cm}}{All Technologies and commodity flows are represented in \autoref{fig:All_RREHs}}\\
\hline
$\mathcal{C}$ &  Electricity, $H_2$, $H_2O$, $CO_2$, and $CH_4$ & Electricity, $H_2$, $H_2O$, $CO_2$, and $CH_3OH$ & Electricity, $H_2$, $H_2O$ & Electricity, $H_2$, $H_2O$, $N_2$, and $NH_3$\\
\hline
$\mathcal{I}$ &  \multicolumn{4}{p{12cm}}{These hubs does not need any direct import or exchange from another systems. Their feed stocks are air and sea water}.\\ 
\hline
$\mathcal{E}$ &  $CH_4$   &  $CH_3OH$   &  $H_2$  & $NH_3$\\
\hline
$\mathcal{B}$ & \multicolumn{3}{|p{9cm}|}{Heat and Oxygen. Where the heat is generated by exothermic process and the oxygen comes from PEM electrolyser.} & In addition to heat and oxygen, a third by-product is argon ($Ar$). Which is produced by the ASU.\\ 
\hline
$\mathcal{O}$ &  \multicolumn{3}{|p{9cm}|}{The integration of desalination units within urban water supply networks ensures a dependable source of drinking water, even in the face of changing climate patterns and population growth.} & In addition to the desalination unit, the generated ammonia can contribute to the development of local agriculture. 

\end{tabular}
\caption{Table characterizing the different RREHs according to the taxonomy presented by citet{}}
\label{tab:taxo}
\end{table*}
